On the Robustness of LLM-Based Dense Retrievers: A Systematic Analysis of Generalizability and Stability

Decoder-only large language models (LLMs) are increasingly replacing BERT-style architectures as the backbone for dense retrieval, achieving substantial performance gains and broad adoption. However, the robustness of these LLM-based retrievers remains underexplored. In this paper, we present the first systematic study of the robustness of state-of-the-art open-source LLM-based dense retrievers from two complementary perspectives: generalizability and stability. For generalizability, we evaluate retrieval effectiveness across four benchmarks spanning 30 datasets, using linear mixed-effects models to estimate marginal mean performance and disentangle intrinsic model capability from dataset heterogeneity. Our analysis reveals that while instruction-tuned models generally excel, those optimized for complex reasoning often suffer a ``specialization tax,'' exhibiting limited generalizability in broader contexts. For stability, we assess model resilience against both unintentional query variations~(e.g., paraphrasing, typos) and malicious adversarial attacks~(e.g., corpus poisoning). We find that LLM-based retrievers show improved robustness against typos and corpus poisoning compared to encoder-only baselines, yet remain vulnerable to semantic perturbations like synonymizing. Further analysis shows that embedding geometry (e.g., angular uniformity) provides predictive signals for lexical stability and suggests that scaling model size generally improves robustness. These findings inform future robustness-aware retriever design and principled benchmarking. Our code is publicly available at https://github.com/liyongkang123/Robust_LLM_Retriever_Eval.

==> Table/general_results_color.tex <==
% \setlength{\arrayrulewidth}{0.1mm} % 调整横线的粗细

\begin{table*}[t]
\centering
% \small
\caption{Experiments results. old Results} 
\label{tab: rq1 Experiments results}
\renewcommand\arraystretch{1} % 
\setlength{\tabcolsep}{1mm}{ % 
\begin{tabular}{l|c |c c|ccccccc}
% \toprule
\hline
% \thickhline
    \multirow{2}{*}{\textbf{Dataset}} & & \multicolumn{2}{c}{\textbf{Instruction-free}}& \multicolumn{5}{c}{\textbf{Instruction-augmented}} \\ \cmidrule(lr){3-4} \cmidrule(lr){5-9} &\textbf{BM25}   & \textbf{Contriever}  &\textbf{BGE-M3} & \textbf{Qwen3} & \textbf{Linq} & \textbf{GTE} & \textbf{ReasonIR} &\textbf{DIVER}  \\
\hline
TREC-COVID   & 65.6   & 59.4 &55.0 &\textbf{94.8} &82.8 &81.1 &76.7 &77.1 &        \\
NFCorpus  &32.5    &32.8 &31.4 &\textbf{41.5} &39.4 &40.1 &37.4 &38.1 &        \\
HotpotQA      & 60.3   &63.8 &69.4 &76.8 &71.5 &73.1 &62.9 &65.8 &        \\
FiQA     & 23.6    &33.0 &41.4 &\textbf{64.7} &53.9 &61.8   &48.2 &48.1        \\
ArguAna      & 31.5   & 44.5 &54.1 &\textbf{76.7} &56.6 &68.5 &60.2 &48.5 &        \\
Quora        & 78.9   &86.4 &88.6 &89.1 &87.3 &\textbf{89.6} &80.9 &88.4 &        \\
DBPedia     &  31.3  & 41.3& 39.8 &49.9 &48.2 &52.4 &39.3 &41.4 &        \\
SCIDOCS      & 15.8  &16.6 & 16.4 &\textbf{32.8} &20.2 &28.9 &22.5 &23.5 &        \\
NQ & 32.9  &49.8 & 60.6&65.1 &67.2 &66.8 &52.9 & 54.2       \\
FEVER   & 75.3    &75.8 &81.4 &91.8 &89.5 &95.2 &76.6 &78.0 &        \\
Climate-FEVER    & 21.3       &23.7 &29.5 &47.4 &53.1 &54.6 &31.7 &30.0 &        \\
SciFact   &  66.5    &67.7 &64.7 &78.4 &77.2 &\textbf{79.4} &75.2 &76.2 &        \\
Touché-2020     & \textbf{36.7}        &20.5 &22.8 &35.0 &26.1 &33.6 &19.8 &24.4 &        \\
\hline
\multicolumn{1}{c}{\textbf{BEIR Avg.}}  &44.0 &47.3 &50.4 &\textbf{64.9} &59.5 &63.5 &52.6 &53.4  \\
\hline
Biology &18.9   &19.0 &9.5 &19.7 &23.1 &30.2 &26.2 & \textbf{42.8}&        \\
Earth Science &27.2  &28.3 &13.7 &32.3 &24.3 &41.1 &31.4 &\textbf{44.4} &        \\
Economics & 14.9    & 17.4 &11.9 &18.2 &17.5 &14.4 &\textbf{23.5} &22.4 &        \\
 Psychology & 12.5    &16.2 &13.5 &25.8 &24.1 &26.8 &30.2 &\textbf{35.3} &        \\
Robotics & 13.6    &14.1 &12.1 &15.3 &13.7 &13.5 &18.2 &\textbf{21.4} &        \\
Stack Overflow &   18.4  &14.2 &10.7 &18.7 &15.1 &16.3 &\textbf{24.0} &21.4 &        \\
 Sustainable Living & 15.0   &14.3 &10.4 &17.5 &21.1 &20.6 &19.8 &\textbf{26.1} &        \\
LeetCode  & 24.4    &22.2 &24.7 &34.1 &31.4 &30.6 &34.6 &\textbf{37.8} &        \\
Pony &7.9     &9.8 &15.1 &0.8 &\textbf{49.6} &2.1 &10.1 &11.7 &        \\
AoPS  &6.2    &9.8 &4.4 &9.4 &4.5 &\textbf{15.7} &15.0 &11.2 &        \\
TheoremQA-Q & 10.4    &10.1 &12.6 &\textbf{39.0} &26.9 &32.3 &31.7 &38.1 &        \\
TheoremQA-T  & 4.9    &4.0 &4.4 &\textbf{38.4} &34.1 &34.4 &27.9 & {37.1} &        \\
\hline
\multicolumn{1}{c}{\textbf{Bright Avg.}} &14.5 &15.0 &11.9 &22.4 &23.8 &23.2 &24.4 &\textbf{29.1}  \\
\hline
 Evidence &1.6  &6.8 &5.7 &\textbf{20.1} &5.4 &17.4 &15.6 &17.7 &        \\
 Gold &1.7     &6.3 &4.9 &\textbf{18.9} &4.1 &17.8 &13.7 &17.3 &        \\
 \hline
\multicolumn{1}{c}{\textbf{BrowseComp-Plus Avg.}}  &1.7 &6.6 &5.3 &19.5 &4.8 &17.6 &14.7 &17.5  \\
\hline
\multicolumn{1}{c}{\textbf{All Avg.}}     &20.1 &22.9 &22.5 &\textbf{35.6} &29.3 &34.7 &30.6 &33.3        \\
\hline
% \bottomrule
\end{tabular}}
\end{table*}


==> Table/general_results_color1.tex <==
% \setlength{\arrayrulewidth}{0.1mm} % 调整横线的粗细

\begin{table*}[t]
\small
\centering
\caption{Experiments results. } 
\label{tab: rq1 Experiments results}
\renewcommand\arraystretch{1} % 
\setlength{\tabcolsep}{0.5mm}{ % 
\begin{tabular}{l|c |c c|ccccccc}
\hline
    \multirow{2}{*}{\textbf{Dataset}} & & \multicolumn{2}{c}{\textbf{Instruction-free}}& \multicolumn{5}{c}{\textbf{Instruction-augmented}} \\ \cmidrule(lr){3-4} \cmidrule(lr){5-9} &\textbf{BM25}   & \textbf{Contriever}  &\textbf{BGE-M3} & \textbf{Qwen3} & \textbf{Linq} & \textbf{GTE} & \textbf{ReasonIR} &\textbf{DIVER}  \\
\hline
TREC-COVID   & 65.6   & 59.4$_{\tiny{-9.4\%}}$ &55.0$_{\tiny{-16.2\%}}$ &\textbf{94.8}$_{\tiny{+44.5\%}}$ &82.8$_{\tiny{+26.3\%}}$ &81.1$_{\tiny{+23.6\%}}$ &76.7$_{\tiny{+16.9\%}}$ &77.1$_{\tiny{+17.5\%}}$ \\
NFCorpus  &32.5    &32.8$_{\tiny{+0.9\%}}$ &31.4$_{\tiny{-3.4\%}}$ &\textbf{41.5}$_{\tiny{+27.7\%}}$ &39.4$_{\tiny{+21.2\%}}$ &40.1$_{\tiny{+23.4\%}}$ &37.4$_{\tiny{+15.1\%}}$ &38.1$_{\tiny{+17.2\%}}$ \\
HotpotQA      & 60.3   &63.8$_{\tiny{+5.8\%}}$ &69.4$_{\tiny{+15.1\%}}$ &76.8$_{\tiny{+27.4\%}}$ &71.5$_{\tiny{+18.6\%}}$ &73.1$_{\tiny{+21.2\%}}$ &62.9$_{\tiny{+4.3\%}}$ &65.8$_{\tiny{+9.1\%}}$ \\
FiQA     & 23.6    &33.0$_{\tiny{+39.8\%}}$ &41.4$_{\tiny{+75.4\%}}$ &\textbf{64.7}$_{\tiny{+174.2\%}}$ &53.9$_{\tiny{+128.4\%}}$ &61.8$_{\tiny{+161.9\%}}$ &48.2$_{\tiny{+104.2\%}}$ &48.1$_{\tiny{+103.8\%}}$ \\
ArguAna      & 31.5   &44.5$_{\tiny{+41.3\%}}$ &54.1$_{\tiny{+71.7\%}}$ &\textbf{76.7}$_{\tiny{+143.8\%}}$ &56.6$_{\tiny{+79.7\%}}$ &68.5$_{\tiny{+117.5\%}}$ &60.2$_{\tiny{+91.1\%}}$ &48.5$_{\tiny{+54.0\%}}$ \\
Quora        & 78.9   &86.4$_{\tiny{+9.5\%}}$ &88.6$_{\tiny{+12.3\%}}$ &89.1$_{\tiny{+12.9\%}}$ &87.3$_{\tiny{+10.7\%}}$ &\textbf{89.6}$_{\tiny{+13.5\%}}$ &80.9$_{\tiny{+2.5\%}}$ &88.4$_{\tiny{+12.0\%}}$ \\
DBPedia     &  31.3  & 41.3$_{\tiny{+31.9\%}}$& 39.8$_{\tiny{+27.2\%}}$ &49.9$_{\tiny{+59.4\%}}$ &48.2$_{\tiny{+54.0\%}}$ &52.4$_{\tiny{+67.4\%}}$ &39.3$_{\tiny{+25.6\%}}$ &41.4$_{\tiny{+32.3\%}}$ \\
SCIDOCS      & 15.8  &16.6$_{\tiny{+5.1\%}}$ & 16.4$_{\tiny{+3.8\%}}$ &\textbf{32.8}$_{\tiny{+107.6\%}}$ &20.2$_{\tiny{+27.8\%}}$ &28.9$_{\tiny{+82.9\%}}$ &22.5$_{\tiny{+42.4\%}}$ &23.5$_{\tiny{+48.7\%}}$ \\
NQ & 32.9  &49.8$_{\tiny{+51.4\%}}$ & 60.6$_{\tiny{+84.3\%}}$ &65.1$_{\tiny{+97.9\%}}$ &67.2$_{\tiny{+104.3\%}}$ &66.8$_{\tiny{+103.0\%}}$ &52.9$_{\tiny{+60.8\%}}$ & 54.2$_{\tiny{+64.7\%}}$ \\
FEVER   & 75.3    &75.8$_{\tiny{+0.7\%}}$ &81.4$_{\tiny{+8.1\%}}$ &91.8$_{\tiny{+21.9\%}}$ &89.5$_{\tiny{+18.8\%}}$ &95.2$_{\tiny{+26.5\%}}$ &76.6$_{\tiny{+1.7\%}}$ &78.0$_{\tiny{+3.6\%}}$ \\
Climate-FEVER    & 21.3       &23.7$_{\tiny{+11.3\%}}$ &29.5$_{\tiny{+38.5\%}}$ &47.4$_{\tiny{+122.5\%}}$ &53.1$_{\tiny{+149.3\%}}$ &54.6$_{\tiny{+156.3\%}}$ &31.7$_{\tiny{+48.8\%}}$ &30.0$_{\tiny{+40.8\%}}$ \\
SciFact   &  66.5    &67.7$_{\tiny{+1.8\%}}$ &64.7$_{\tiny{-2.7\%}}$ &78.4$_{\tiny{+17.9\%}}$ &77.2$_{\tiny{+16.1\%}}$ &\textbf{79.4}$_{\tiny{+19.4\%}}$ &75.2$_{\tiny{+13.1\%}}$ &76.2$_{\tiny{+14.6\%}}$ \\
Touché-2020     & \textbf{36.7}        &20.5$_{\tiny{-44.1\%}}$ &22.8$_{\tiny{-37.9\%}}$ &35.0$_{\tiny{-4.6\%}}$ &26.1$_{\tiny{-28.8\%}}$ &33.6$_{\tiny{-8.4\%}}$ &19.8$_{\tiny{-46.0\%}}$ &24.4$_{\tiny{-33.5\%}}$ \\
\hline
\multicolumn{1}{c}{\textbf{BEIR Avg.}}  &44.0 &47.3$_{\tiny{+7.5\%}}$ &50.4$_{\tiny{+14.5\%}}$ &\textbf{64.9}$_{\tiny{+47.5\%}}$ &59.5$_{\tiny{+35.2\%}}$ &63.5$_{\tiny{+44.3\%}}$ &52.6$_{\tiny{+19.5\%}}$ &53.4$_{\tiny{+21.4\%}}$  \\
\hline
Biology &18.9   &19.0$_{\tiny{+0.5\%}}$ &9.5$_{\tiny{-49.7\%}}$ &19.7$_{\tiny{+4.2\%}}$ &23.1$_{\tiny{+22.2\%}}$ &30.2$_{\tiny{+59.8\%}}$ &26.2$_{\tiny{+38.6\%}}$ & \textbf{42.8}$_{\tiny{+126.5\%}}$ \\
Earth Science &27.2  &28.3$_{\tiny{+4.0\%}}$ &13.7$_{\tiny{-49.6\%}}$ &32.3$_{\tiny{+18.8\%}}$ &24.3$_{\tiny{-10.7\%}}$ &41.1$_{\tiny{+51.1\%}}$ &31.4$_{\tiny{+15.4\%}}$ &\textbf{44.4}$_{\tiny{+63.2\%}}$ \\
Economics & 14.9    & 17.4$_{\tiny{+16.8\%}}$ &11.9$_{\tiny{-20.1\%}}$ &18.2$_{\tiny{+22.1\%}}$ &17.5$_{\tiny{+17.4\%}}$ &14.4$_{\tiny{-3.4\%}}$ &\textbf{23.5}$_{\tiny{+57.7\%}}$ &22.4$_{\tiny{+50.3\%}}$ \\
Psychology & 12.5    &16.2$_{\tiny{+29.6\%}}$ &13.5$_{\tiny{+8.0\%}}$ &25.8$_{\tiny{+106.4\%}}$ &24.1$_{\tiny{+92.8\%}}$ &26.8$_{\tiny{+114.4\%}}$ &30.2$_{\tiny{+141.6\%}}$ &\textbf{35.3}$_{\tiny{+182.4\%}}$ \\
Robotics & 13.6    &14.1$_{\tiny{+3.7\%}}$ &12.1$_{\tiny{-11.0\%}}$ &15.3$_{\tiny{+12.5\%}}$ &13.7$_{\tiny{+0.7\%}}$ &13.5$_{\tiny{-0.7\%}}$ &18.2$_{\tiny{+33.8\%}}$ &\textbf{21.4}$_{\tiny{+57.4\%}}$ \\
Stack Overflow &   18.4  &14.2$_{\tiny{-22.8\%}}$ &10.7$_{\tiny{-41.8\%}}$ &18.7$_{\tiny{+1.6\%}}$ &15.1$_{\tiny{-17.9\%}}$ &16.3$_{\tiny{-11.4\%}}$ &\textbf{24.0}$_{\tiny{+30.4\%}}$ &21.4$_{\tiny{+16.3\%}}$ \\
Sustainable Living & 15.0   &14.3$_{\tiny{-4.7\%}}$ &10.4$_{\tiny{-30.7\%}}$ &17.5$_{\tiny{+16.7\%}}$ &21.1$_{\tiny{+40.7\%}}$ &20.6$_{\tiny{+37.3\%}}$ &19.8$_{\tiny{+32.0\%}}$ &\textbf{26.1}$_{\tiny{+74.0\%}}$ \\
LeetCode  & 24.4    &22.2$_{\tiny{-9.0\%}}$ &24.7$_{\tiny{+1.2\%}}$ &34.1$_{\tiny{+39.8\%}}$ &31.4$_{\tiny{+28.7\%}}$ &30.6$_{\tiny{+25.4\%}}$ &34.6$_{\tiny{+41.8\%}}$ &\textbf{37.8}$_{\tiny{+55.0\%}}$ \\
Pony &7.9     &9.8$_{\tiny{+24.1\%}}$ &15.1$_{\tiny{+91.1\%}}$ &0.8$_{\tiny{-89.9\%}}$ &\textbf{49.6}$_{\tiny{+528.0\%}}$ &2.1$_{\tiny{-73.4\%}}$ &10.1$_{\tiny{+27.8\%}}$ &11.7$_{\tiny{+48.1\%}}$ \\
AoPS  &6.2    &9.8$_{\tiny{+58.1\%}}$ &4.4$_{\tiny{-29.0\%}}$ &9.4$_{\tiny{+51.6\%}}$ &4.5$_{\tiny{-27.4\%}}$ &\textbf{15.7}$_{\tiny{+153.2\%}}$ &15.0$_{\tiny{+141.9\%}}$ &11.2$_{\tiny{+80.6\%}}$ \\
TheoremQA-Q & 10.4    &10.1$_{\tiny{-2.9\%}}$ &12.6$_{\tiny{+21.2\%}}$ &\textbf{39.0}$_{\tiny{+275.0\%}}$ &26.9$_{\tiny{+158.7\%}}$ &32.3$_{\tiny{+210.6\%}}$ &31.7$_{\tiny{+204.8\%}}$ &38.1$_{\tiny{+266.3\%}}$ \\
TheoremQA-T  & 4.9    &4.0$_{\tiny{-18.4\%}}$ &4.4$_{\tiny{-10.2\%}}$ &\textbf{38.4}$_{\tiny{+683.7\%}}$ &34.1$_{\tiny{+595.9\%}}$ &34.4$_{\tiny{+602.0\%}}$ &27.9$_{\tiny{+469.4\%}}$ & {37.1}$_{\tiny{+657.1\%}}$ \\
\hline
\multicolumn{1}{c}{\textbf{Bright Avg.}} &14.5 &15.0$_{\tiny{+3.4\%}}$ &11.9$_{\tiny{-17.9\%}}$ &22.4$_{\tiny{+54.5\%}}$ &23.8$_{\tiny{+64.1\%}}$ &23.2$_{\tiny{+60.0\%}}$ &24.4$_{\tiny{+68.3\%}}$ &\textbf{29.1}$_{\tiny{+100.7\%}}$  \\
\hline
 Evidence &1.6  &6.8$_{\tiny{+325.0\%}}$ &5.7$_{\tiny{+256.3\%}}$ &\textbf{20.1}$_{\tiny{+1156.3\%}}$ &5.4$_{\tiny{+237.5\%}}$ &17.4$_{\tiny{+987.5\%}}$ &15.6$_{\tiny{+875.0\%}}$ &17.7$_{\tiny{+1006.3\%}}$ \\
 Gold &1.7     &6.3$_{\tiny{+270.6\%}}$ &4.9$_{\tiny{+188.2\%}}$ &\textbf{18.9}$_{\tiny{+1011.8\%}}$ &4.1$_{\tiny{+141.2\%}}$ &17.8$_{\tiny{+947.1\%}}$ &13.7$_{\tiny{+705.9\%}}$ &17.3$_{\tiny{+917.6\%}}$ \\
 \hline
\multicolumn{1}{c}{\textbf{BrowseComp-Plus Avg.}}  &1.7 &6.6$_{\tiny{+288.2\%}}$ &5.3$_{\tiny{+211.8\%}}$ &19.5$_{\tiny{+1047.1\%}}$ &4.8$_{\tiny{+182.4\%}}$ &17.6$_{\tiny{+935.3\%}}$ &14.7$_{\tiny{+764.7\%}}$ &17.5$_{\tiny{+929.4\%}}$  \\
\hline
\multicolumn{1}{c}{\textbf{All Avg.}}     &20.1 &22.9$_{\tiny{+13.9\%}}$ &22.5$_{\tiny{+11.9\%}}$ &\textbf{35.6}$_{\tiny{+77.1\%}}$ &29.3$_{\tiny{+45.8\%}}$ &34.7$_{\tiny{+72.6\%}}$ &30.6$_{\tiny{+52.2\%}}$ &33.3$_{\tiny{+65.7\%}}$        \\
\hline
\end{tabular}}
\end{table*}


==> Table/general_results_old.tex <==
% % \setlength{\arrayrulewidth}{0.1mm} % 调整横线的粗细

% \begin{table*}[t]
% \centering
% \small
% \renewcommand\arraystretch{1} % 
% \setlength{\tabcolsep}{1mm}{ % 
% \begin{tabular}{l|c |c c|ccccccc}
% % \toprule
% \hline
% % \thickhline
%     \multirow{2}{*}{\textbf{Dataset}} & & \multicolumn{2}{c}{\textbf{Instruction-free}}& \multicolumn{6}{c}{\textbf{Instruction-augmented}} \\ \cmidrule(lr){3-4} \cmidrule(lr){5-10} &\textbf{BM25}   & \textbf{Contriever}  &\textbf{BGE-M3} & \textbf{Qwen3} & \textbf{Linq} & \textbf{GTE} & \textbf{ReasonIR} &\textbf{DIVER} &  \textbf{ReasonEmbed} \\
% \hline
% TREC-COVID   & 65.6   & {59.4} &55.0 &\textbf{94.8} &82.8 &81.1 &76.7 &77.1 &        \\
% NFCorpus  &32.5    &32.8 &31.4 &\textbf{41.5} &39.4 &40.1 &37.4 &38.1 &        \\
% HotpotQA      & 60.3   &63.8 &69.4 &\textbf{76.8} &71.5 &73.1 &62.9 &65.8 &        \\
% FiQA     & 23.6    &33.0 &41.4 &\textbf{64.7} &53.9 &61.8   &48.2 &48.1        \\
% ArguAna      & 31.5   & 44.5 &54.1 &\textbf{76.7} &56.6 &68.5 &60.2 &48.5 &        \\
% Quora        & 78.9   &86.4 &88.6 &89.1 &87.3 &\textbf{89.6} &80.9 &88.4 &        \\
% DBPedia     &  31.3  & 41.3& 39.8 &49.9 &48.2 &52.4 &39.3 &41.4 &        \\
% SCIDOCS      & 15.8  &16.6 & 16.4 &\textbf{32.8} &20.2 &28.9 &22.5 &23.5 &        \\
% NQ & 32.9  &49.8 & 60.6&65.1 &67.2 &66.8 &52.9 & 54.2       \\
% FEVER   & 75.3    &75.8 &81.4 &91.8 &89.5 &95.2 &76.6 &78.0 &        \\
% Climate-FEVER    & 21.3       &23.7 &29.5 &47.4 &53.1 &54.6 &31.7 &30.0 &        \\
% SciFact   &  66.5    &67.7 &64.7 &78.4 &77.2 &\textbf{79.4} &75.2 &76.2 &        \\
% Touché-2020     & \textbf{36.7}        &20.5 &22.8 &35.0 &26.1 &33.6 &19.8 &24.4 &        \\
% \hline
% \multicolumn{1}{c}{\textbf{BEIR Avg.}}  &44.0 &47.3 &50.4 &\textbf{64.9} &59.5 &63.5 &52.6 &53.4  \\
% \hline
% Biology &18.9   &19.0 &9.5 &19.7 &23.1 &30.2 &26.2 & \textbf{42.8}&        \\
% Earth Science &27.2  &28.3 &13.7 &32.3 &24.3 &41.1 &31.4 &\textbf{44.4} &        \\
% Economics & 14.9    & 17.4 &11.9 &18.2 &17.5 &14.4 &\textbf{23.5} &22.4 &        \\
%  Psychology & 12.5    &16.2 &13.5 &25.8 &24.1 &26.8 &30.2 &\textbf{35.3} &        \\
% Robotics & 13.6    &14.1 &12.1 &15.3 &13.7 &13.5 &18.2 &\textbf{21.4} &        \\
% Stack Overflow &   18.4  &14.2 &10.7 &18.7 &15.1 &16.3 &\textbf{24.0} &21.4 &        \\
%  Sustainable Living & 15.0   &14.3 &10.4 &17.5 &21.1 &20.6 &19.8 &\textbf{26.1} &        \\
% LeetCode  & 24.4    &22.2 &24.7 &34.1 &31.4 &30.6 &34.6 &\textbf{37.8} &        \\
% Pony &7.9     &9.8 &15.1 &0.8 &\textbf{49.6} &2.1 &10.1 &11.7 &        \\
% AoPS  &6.2    &9.8 &4.4 &9.4 &4.5 &\textbf{15.7} &15.0 &11.2 &        \\
% TheoremQA-Q & 10.4    &10.1 &12.6 &\textbf{39.0} &26.9 &32.3 &31.7 &38.1 &        \\
% TheoremQA-T  & 4.9    &4.0 &4.4 &\textbf{38.4} &34.1 &34.4 &27.9 & {37.1} &        \\
% \hline
% \multicolumn{1}{c}{\textbf{Bright Avg.}} &14.5 &15.0 &11.9 &22.4 &23.8 &23.2 &24.4 &\textbf{29.1}  \\
% \hline
%  Evidence &1.6  &6.8 &5.7 &\textbf{20.1} &5.4 &17.4 &15.6 &17.7 &        \\
%  Gold &1.7     &6.3 &4.9 &\textbf{18.9} &4.1 &17.8 &13.7 &17.3 &        \\
%  \hline
% \multicolumn{1}{c}{\textbf{BrowseComp-Plus Avg.}}  &1.7 &6.6 &5.3 &19.5 &4.8 &17.6 &14.7 &17.5  \\
% \hline
% \multicolumn{1}{c}{\textbf{All Avg.}}     &20.1 &22.9 &22.5 &\textbf{35.6} &29.3 &34.7 &30.6 &33.3        \\
% \hline
% % \bottomrule
% \end{tabular}}
% \caption{Experiments results, nDCG@10.} 
% \label{tab: rq1 Experiments results}
% \end{table*}

==> Table/query_specific_results_average.tex <==
\begin{table*}[t]
\centering
\small
\caption{Micro-averaged nDCG@10 by task type, query type, and corpus source type. Scores are computed by directly averaging query-level results without controlling for dataset difficulty (cf. EMMs in Table~\ref{tab:emm_merge_results}).}
\label{tab:raw_mean_results}
\renewcommand\arraystretch{1.0}
\setlength{\tabcolsep}{1.5pt}
\begin{tabular}{llccccccccccccc}
\toprule
\multirow{2}{*}{\textbf{Factor}}&\multirow{2}{*}{\textbf{Level}} &
  & \multicolumn{2}{c}{\textbf{Instruction-free}} 
  & \multicolumn{6}{c}{\textbf{Instruction-augmented}} \\
\cmidrule(lr){4-5} \cmidrule(lr){6-11}
& & \textbf{BM25} & \textbf{Contriever} & \textbf{BGE-M3} 
 & \textbf{Qwen3} & \textbf{Linq} & \textbf{GTE} & \textbf{ReasonIR} & \textbf{DIVER} & \textbf{ReasonEmbed}   \\
\midrule
% \multicolumn{10}{l}{\textit{Task types}} \\
 
\multirow{11}{*}{\shortstack[l]{Task \\Type }}
&Passage Retrieval & 22.1  & 41.1  &38.8    &44.2    &45.3    &46.3   & 32.7  &31.9   &  32.7  \\
&Bio-Medical Retrieval   & 34.3  & 36.4 & 34.9  & 48.5  & 48.0  & 45.5 & 43.1  & 43.5  & 45.4      \\
&Question Answering  &45.9   & 54.4  & 61.2   & 69.0   &69.6    &67.0   & 56.0  &58.4   &47.1      \\
&Duplicate Question Retrieval &76.9   &86.4  & 88.6  & 89.0  & 90.2 & 89.6 & 81.0  & 88.4  &48.5   \\
&Entity-Retrieval    &31.0   & 41.3 & 39.8  & 50.0  &51.3 & 52.4  & 39.7 & 41.5 &41.3 \\
&Citation-Prediction  & 14.4  &16.6  & 16.4  & 32.8   & 22.1  & 28.9 &22.8  & 23.5  &22.5      \\
&Fact Checking &52.4   &66.1  & 71.1  &83.3   &82.3  & 85.8  & 69.1  & 69.2 & 58.4   \\
&Argument Retrieval   & 38.9   & 43.7 & 52.9  & 75.3  & 66.9 & 67.3 & 58.9  & 47.5  & 48.3 \\
&StackExchange Post Retrieval   &17.4   & 17.7 &12.0   & 21.5  &23.7  &23.3 & 24.8  &30.1  &43.4 \\
&Code Retrieval &16.9  & 16.7  & 20.3  & 19.4  &27.7 &18.4 &23.5  & 27.1 & 27.0    \\
&Theorem Retrieval   &8.1   & 8.8 & 8.9  &30.5 &  23.7 &28.1  &25.9  &30.2  &  33.8   \\
% \cdashline{1-10}
\hdashline
&Avg. (task)    &     32.6& 39.0& 40.4& 51.2&50.1&50.2&43.4 &44.7&40.8   \\

\midrule
% \multicolumn{10}{l}{\textit{Query types}} \\
 
\multirow{9}{*}{\shortstack[l]{Query \\Type }}
&FACTOID   &42.5  &52.5  &56.3  &63.3   &63.9  &62.5    & 50.9  &53.1  &44.2  \\
&INSTRUCTION  & 62.8 & 72.4  &75.0  & 77.4  &78.4  & 78.4   &67.4   &75.4  &36.9  \\
&REASON & 64.0 & 73.3 &75.3  & 78.2  &79.8  & 78.7   &72.9   &76.8  &50.2  \\
&EVIDENCE-BASED   & 39.7 & 55.8  &56.0  & 60.6  &61.3  & 61.8   &51.8   &52.1  & 38.5 \\
&COMPARISON  & 70.4 &81.6  &85.9  &88.7   & 89.3 & 87.6   & 78.4  & 82.3 & 59.6 \\
&EXPERIENCE & 73.7 &84.0  &86.8  & 87.2  &88.8  &  88.0  & 77.2  & 86.7 & 44.6 \\
&DEBATE   & 67.2 &76.1 &78.9  & 82.7  &83.2  & 82.4   & 73.3  & 78.6 &52.5  \\
&NOT-A-QUESTION   &45.2  &56.1  &60.7  &74.1   &71.9  & 74.5   & 61.4  &60.5  & 52.8 \\
% \cdashline{1-10}
\hdashline
&Avg. (query)  & 58.2&69.0&71.9&76.5&77.1&76.7&66.7&70.7&47.4       \\
\midrule
% \multicolumn{10}{l}{\textit{Corpus Source types}} \\
\multirow{6}{*}{\shortstack[l]{Corpus\\Source\\Type}}
&General Web     & 20.3      & 37.5     & 35.4    & 41.6    & 41.8    & 43.3   & 30.9    & 30.4     & 31.0        \\
&Scientific Paper  &28.3      &30.2     & 29.1    & 44.5    & 38.0    & 41.7  &36.7     &  37.4   &37.7         \\
&Wikipedia  & 50.6      & 61.8   & 68.1    & 77.0    & 77.4     & 77.0 &63.1    & 64.5    & 52.8        \\
&Online Community  &  70.0     &78.9     & 80.8   & 83.2    & 84.2    &86.7   & 75.5    & 82.2    &  47.9       \\
&Domain KB  & 30.6      & 34.1    & 41.0    & 60.3    & 54.2    & 54.2  &  48.6   & 41.9    &43.0         \\
% \cdashline{1-10}
\hdashline
&Avg. (corpus source)           & 40.0 &48.5 &50.9 &61.3 &59.1 &60.6 &51.0 &51.3 &42.5   \\
\bottomrule
\end{tabular}
\end{table*}

